Staggered schemes for compressible flow: a general construction

This paper is focused on the approximation of the Euler equations of compressible fluid dynamics on a staggered mesh. With this aim, the flow parameters are described by the velocity, the density and the internal energy. The thermodynamic quantities are described on the elements of the mesh, and thus the approximation is only in $L^2$, while the kinematic quantities are globally continuous. The method is general in the sense that the thermodynamic and kinetic parameters are described by an arbitrary degree of polynomials. In practice, the difference between the degrees of the kinematic parameters and the thermodynamic ones {is set} to $1$. The integration in time is done using the forward Euler method but can be extended straightforwardly to higher-order methods. In order to guarantee that the limit solution will be a weak solution of the problem, we introduce a general correction method in the spirit of the Lagrangian staggered method described in \cite{Svetlana,MR4059382, MR3023731}, and we prove a Lax Wendroff theorem. The proof is valid for multidimensional versions of the scheme, even though most of the numerical illustrations in this work, on classical benchmark problems, are one-dimensional because we have easy access to the exact solution for comparison. We conclude by explaining that the method is general and can be used in different settings, for example, Finite Volume, or discontinuous Galerkin method, not just the specific one presented in this paper.

==> command.tex <==
\usepackage{fullpage}

\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{mathrsfs}
\usepackage{color,xcolor}
\usepackage{ifpdf}
\usepackage{psfrag}
\usepackage{graphicx,graphics,subfigure,epsfig}
\usepackage{url}
\usepackage{hyperref}
%\usepackage{showkeys}
\usepackage{xspace}
\usepackage{nicefrac}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corrolary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{lemme}[theorem]{Lemma}
\newtheorem{exemple}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remarque}[theorem]{Remark}
%\theoremstyle{remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dpar}[2]{\dfrac{\partial #1}{\partial #2}}

\renewcommand{\div}{\text{ div }}
\newcommand{\burb}{~These results have been obtained by  A. Burbeau \cite{burbeau} and reproduced with  permission.}

 \newcommand{\R}{\mathbb R}
 \newcommand{\Z}{\mathbb Z}
 \newcommand{\N}{\mathbb N}
 \newcommand{\C}{\mathbb C}
 \newcommand{\Q}{\mathbb Q}
 \newcommand{\K}{\mathbb K}
\renewcommand{\P}{\mathbb P}
\newcommand{\CC}{\mathcal{C}}
 
\newcommand{\PP}{\mathbb P}
\newcommand{\QQ}{\mathcal Q}


\newcommand{\TT}{\mathcal{T}}
\renewcommand{\SS}{\mathcal{S}}
%\newcommand{\SSS}{\mathcal{S}}


\newcommand{\ds}{DS}
\newcommand{\T}{\mathcal{T}}
\newcommand{\LL}{\mathcal{L}}
\renewcommand{\SS}{\mathcal{S}}
\newcommand{\KK}{\mathcal K}
\newcommand{\Id}{\text{Id }}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\BW}{U}

\newcommand{\bbf}{{\mathbf {f}}}
\newcommand{\bn}{{\mathbf {n}}}
\newcommand{\bm}{\mathbf{m}}


\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bq}{\mathbf{q}}

\newcommand{\Uq}{\underline{\mathbf{q}}}

\newcommand{\bF}{\mathbf{f}}
\newcommand{\bbF}{\mathbf{\mathcal{F}}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bbu}{\mathbf{u}}
\newcommand{\bbg}{\mathbf{g}}
\newcommand{\hbbg}{\hat{\mathbf{g}}}
\newcommand{\hbbf}{\hat{\mathbf{f}}}
\newcommand{\hf}{\hat{\mathbf{f}}}
\newcommand{\hh}{\hat{f}}
\newcommand{\saut}[1]{\big [ #1 \big ]}
\newcommand{\moy}[1]{\big\{#1\big\}}


\newcommand{\ba}{\mathbf{a}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bvit}{\mathbf{u}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\ICI}{\red{\large{ICI}}}

%%
\newcommand{\buscal}{u}
\newcommand{\bvscal}{v}

\newcommand{\ent}{\eta}
\newcommand{\enf}{q}


\newcommand{\normal}{\mathbf{N}}

%\newcommand{\bbf}{{\mathbf {f}}}
\newcommand{\bxx}{{\mathbf {x}}}
%\newcommand{\bn}{{\mathbf {n}}}
\newcommand{\s}{\sqrt{2}}
\newcommand{\is}{\frac{\sqrt{2}}{2}}
%\newcommand{\hf}{\hat{f}}
\newcommand{\Bf}{\mathbf{f}}
%\newcommand{\dpar}[2]{\dfrac{\partial #1}{\partial #2}}


%\newcommand{\bu}{u}%\mathbf{u}}
%\newcommand{\bv}{v}%\mathbf{v}}
\newcommand{\Bv}{\undeline{v}}%\underline{\mathbf{v}}}

\newcommand{\bbv}{v}%\mathbf{v}}

\newcommand{\Bbv}{\underline{\mathbf{v}}}

%\newcommand{\bF}{\mathbf{f}}
%\newcommand{\bbF}{\mathbf{\mathcal{F}}}
%\newcommand{\bK}{\mathbf{K}}
%\newcommand{\bbu}{u}%\mathbf{u}}
%\newcommand{\bbg}{\mathbf{g}}
%\newcommand{\hbbg}{\hat{\mathbf{g}}}
%\newcommand{\hbbf}{\hat{\mathbf{f}}}

%\newcommand{\ba}{\mathbf{a}}
%\newcommand{\bx}{\mathbf{x}}
%\newcommand{\by}{\mathbf{y}}
%
%\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\ICI}{\red{\large{ICI}}}
%
\newcommand{\norm}[1]{\big |\big | #1\big |\big |}
\newcommand{\abs}[1]{\big | #1\big |}
\newcommand{\diver}{\text{div }}
%%%%%%%%%%%%%%%


==> convergence.tex <==
\appendix
%\section{B\'ezier polynomials: notations}\label{sec:Bezier}
%If $K$ is a simplex, we will denote its vertices as $v$, or $v_i$, or $i$, knowing that we have $d+1$ vertices. The barycentric coordinates with respect to the vertices will be denoted by $\lambda_v$ or $\lambda_i$, depending on the context. The B\'ezier polynomials of degree $n$ are labelled according to a  multi-index with $d+1$ components, $(k_1, \ldots , k_{d+1})$ with $\sum_{i=1}^{d+1} k_i=n$, or a degree of freedom $\sigma$ according to the context. To fix ideas, let is detail the 2D case. The B\'ezier polynomial of index $(k_1,k_2,k_3)$  corresponds to the degree of freedom $\sigma$ that we identify to the point $\bx_\sigma$ in $K$ which barycentric coordinates are $(\tfrac{k_1}{n}, \tfrac{k_2}{n}, \tfrac{k_3}{n})$ which are called the Greville points. We have
%$$B_{k_1,k_2,k_3}:=\dfrac{k_1! k_2!k_3!}{(k_1+k_2+k_3)!}\lambda_1^{k_1}\lambda_2^{k_2}\lambda_3^{k_3}:=B_\sigma$$
%and we see that
%\begin{itemize}
%\item 
%$\sum_{\sigma\in K}B_\sigma=\sum_{k_i\geq 0, k_1+k_2+k_3=n} B_{(k_1,k_2,k_3)}=1$,
%\item $B_\sigma\geq 0$ on $K$,
%\item
%$$\int_K B_{k_1,k_2,k_3}(\bx)\; d\bx=\dfrac{2}{(n+1)(n+2)} |K|.$$
%\end{itemize}
%The B\'ezier polynomials of degree $n$ constitute a basis of $\P^n$, the set of polynomials of degree less or equal to $n$. 
%
%We have:
%\begin{itemize}
%\item $k=1$, $B_{100}=\lambda_1$, $B_{010}=\lambda_2$, $B_{001}=\lambda_3$,
%\item $k=2$, $B_{200}=\lambda_1^2$, $B_{020}=\lambda_2^2$,$B_{002}=\lambda_3^2$, $B_{110}=2\lambda_1\lambda_2$,  $B_{101}=2\lambda_1\lambda_3$, $B_{011}=2\lambda_2\lambda_3$, 
%\item $k=3$, 
%$B_{300}=\lambda_1^3$, $B_{030}=\lambda_2^3$, $B_{003}=\lambda_3^3$, $B_{210}=3\lambda_1^2\lambda_2$, $B_{120}=3\lambda_1\lambda_2^2$, $B_{021}=3\lambda_2^2\lambda_3$, $B_{012}=3\lambda_1\lambda_2^2$, $B_{201}=3\lambda_1^2\lambda_3$, $B_{102}=3\lambda_1\lambda_3$, $B_{111}=6\lambda_1\lambda_2\lambda_3$.
%\end{itemize}
%
\section{Lax-Wendroff like result}\label{LxWthm}
\subsection{Notations and basic concepts}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We explain our notations, and specify the degrees of freedom. In a mesh 
$\mathcal{T}$ whose elements are denoted by $K$. 
We seek a solution that is piecewise polynomial of degree $k$ in each 
element, and therefore need to provide each $K$ with $(k+1)(k+2)/2$ 
degrees of freedom; these degrees of freedom will genericaly be denoted by $\sigma$. A simple way to do this is to use $\P^k$ elements whose 
degrees of freedom are the values of the solution at the points whose 
barycentric coordinates within $K$ are $\{i/k,j/k,(k-i-j)/k\}$ for $0\leq
 i , j \le k$. 






For any element $K$, we denote by $h_K$ its diameter, $|K|$ its area and 
$h=\max_{K} h_K$.

The schemes that we study here are of the following form~: 
for any degre of freedom $\sigma$ 
\begin{subequations}
\label{leschema}
\begin{equation}\label{leschema:formule}
u^{n+1}_\sigma= u^{n}_\sigma - \dfrac{\Delta t}{|C_\sigma|} \sum_{K, \sigma \in K} \Psi_\sigma^K
\end{equation}
and the residual satisfy the conservation relation
\begin{equation}\label{leschemea:cons}
\sum\limits_{\sigma \in K}\Phi_\sigma^K(\bu^h)=\int_{\partial K} \bbf^h\cdot \; d\gamma
\end{equation}
\end{subequations}

Here $C_\sigma$ is the dual control volume associated { with the dof $\sigma$}.



\subsection{A Lax Wendroff theorem}\label{sec:lax}
%%%%%%%%%%%%%%%
Under which reasonable conditions can the scheme (\ref{leschema}) converge towards a weak
solution of \eqref{problem}?
 To answer this question, we give a Lax Wendroff--like theorem.
Let us give some conditions on the mesh,  the residuals
$\Phi_\sigma^{K}$, and define some notations and
functional spaces.

\begin{assumption}
\label{H0}
The mesh $\TT_h$ is conformal and regular. By regular we mean that all elements
 are roughly the same size, more 
precisely that there exist  constants 
 $C_1$ and  $C_2$ such that for any element
$$ K, \; \; C_1 \leq \sup_{K \in \mathcal{K}_h} \dfrac{h^2}{|K|} \leq C_2.$$
\end{assumption}
We say that two elements are neighbors if they have a common edge


Let $\TT_h$ be a triangulation satisfying assumption \ref{H0},
 and ${\cal C}_h$ be 
a set of dual volumes
associated with the degrees of freedom $\sigma$. Then we define the 
following subspaces,
$$
\begin{array}{l}
V_h^k=\{ v_h \in C^0(\R^2); {v_{h}}_{|K} \text{ polynomial of degree k }, \forall ~K \in
\TT_h \}\\
~~\\
X^h=\{v_h; {v_h}_{|C} \text{ constant }\in \R^{p}, \forall ~C \in \CC_h\}.
\end{array}
$$
Here, $\bbf_{|K}$ denotes the restriction of $\bbf$ to $K$. The basis functions of $V_h^k$ are $\{\varphi_\sigma\}_{\sigma}$. Since $\P^k$ is finite dimensional, there exist two constants, $C_1>0$ and $C_2>$ depending only on $k$ such that for any $v\in \P^k$, 
\begin{equation}
\label{assumption basis functions}
C_{1}|K|\sum_{\sigma\in K}|v_\sigma| \leq \int_K\big |v\big |\; d\bx\leq C_{2}|K|\sum_{\sigma\in K} |v_\sigma|.
\end{equation}

We denote  by $\pi_h^1v$ the piecewise linear interpolation of a continuous
 function.
Let  $L_h~: V_h^k \rightarrow X^h$ be the mass lumping operator,
$L_h(v)=\sum_\sigma v(x_\sigma) \chi_{\sigma}$ where $\chi_{\sigma}$ is the characteristic 
function of the cell $C_\sigma$.

\bigskip

We assume that the residual 
$\Phi_{\sigma}^{K'_K}$ 
and the numerical solution satisfy the following conditions.
\begin{assumption}
\label{H2} Let $\TT_h$ be a triangulation satisfying  the assumption \ref{H0}.
For any  $C\in \R^+$, there exists $C'( C, \TT_h)\in \R^+$ which depends only on 
$C$ and  $\TT_h$ such that  for any 
$ u \in V_h^k, \text{ with }  \norm{u}_{L^{\infty}(\R^2)}\leq C$  we have 
\begin{equation}
\label{eq:conservation}
\forall K, \forall \sigma, \norm{\Phi_{\sigma}^{K}}\leq C'(C, \TT_h) \; h\;
\sum_{\sigma'\in K}\norm{u_{\sigma'}-u_{\sigma}}.
\end{equation}
\end{assumption}

\begin{remark}
{One should see this assumption as { asserting continuity of the 
residual components (or signals)} $\Phi_\sigma^{K}$ with respect of the 
nodal values of $u$; in particular, when $u$ is constant, 
$\Phi_\sigma^{K}=0$. The proof of Theorem \ref{th1} when  
$\Phi_{\sigma}^{K}$ satisfy  assumption \ref{H2} is still valid if the number of arguments in $\Phi_\sigma^{K}$
is bounded independently of $h$ and the element $K$. In practice,
 this is always true if the triangulation
is uniform, since the arguments of $\Phi_\sigma^{K}$ are contained in some
neighbourhood of $\sigma$ comprising a finite number of points.
}
\end{remark}

\begin{assumption}
\label{H3}
If   ${\hbbf_\bn}$ is a consistent approximation of of the flux  ${\bbf}$ in the direction $\bn$ such that
\begin{enumerate}
\item[(i)] $\forall \bv^h \in V_h^k$, $\Phi^K(\bv^h):=\displaystyle \int_{\partial K}
{\hbbf}^h(\bv^h) \cdot \bn \; d{\gamma}=\sum\limits_{\sigma \in K} \Phi_{\sigma}^{K}(\bv^h),$
\item[(ii)] $\forall \bv^h \in V_h^k$, and for any  $K_1$ and $K_2$ are neighbouring elements,
$${\hbbf}_\bn = -\hbbf_\bn\ \; \; p.p.
\text{ on }
K_1 \cap K_2 $$
where $\bn$ is a normal of  $K_1\cap K_2$.
\item[(iii)] For any  $C>0$, there exists  $C'(C)$ such that for any 
$ \bv^h\in X^h$ with $||\bv^h||_{L^{\infty }({\R}^2)}\leq C $,
{one has for } $  K\in
\TT_h $ and  $ {\bbf}^h_K = {\bbf}^h_{|K}$,
$$\Big | \int_{\partial K} \hbbf_\bn \; d\gamma \Big | \leq 
{h}   \sum \limits_{\sigma,\sigma'\in \mathcal{S}} || \bv_\sigma^h-\bv_{\sigma'}^h ||$$ a.e.
on  $K$. Here $\mathcal{S}$ is the set of all possible degrees of freedom that are needed to evaluate $\int_{\partial K} \hbbf_\bn \; d\gamma$, i.e. this at most the union of all the degrees of freedom attached to $K$ and its neighbors.
\item[(iv)] For any sequence  $(\bv^h)_h$  bounded in 
$L^{\infty}(\R^2 \times \R^{+})^p$
independantly of  $h$ and convergent in  $L^2_{loc}(\R^2 \times \R^+)^p$ to  
$\bv$, we have 
$$\lim_h \norm{ \bbf^h(\bv^h)-\bbf(\bv)}_{L^1_{loc}(\R^2\times \R^+)^p}=0.$$
\end{enumerate}
\end{assumption}


We have the following result,
\begin{theorem}
\label{th1}
Let be  $\bu_0\in L^{\infty}(\R^d)^p$ and 
 $\bu^h$ the approximation given by  (\ref{leschema}). We assume that 
the scheme satisfies 
the assumptions  \ref{H2} and  \ref{H3}. We also assume there exists a constant 
$C$ that depends only on
 $C_1$, $C_2$ and  $u_0$  and a function  $\bu\in (L^2(\R^d \times \R^+))^p$
such that 
$$
\begin{array}{l}
\sup_h \sup_{x,y,t} |\bu^h(x,y,t)|\leq C \\
~\\
\lim_h \norm{\bu-\bu_h}_{L^2_{loc}(\R^d\times \R^+)^p}=0
\end{array}
$$
Then  $\bu$  is a weak solution of  \eqref{problem}.
\end{theorem}
For the
sake of simplicity, we assume $d=2$, the generalisation is immediate.

\bigskip

Last, $\pi_h^k$ is the $\P^k$ interpolation defined on $V_h^k$. 

\medskip

We start by  a lemma that is inspired from  \cite{Kroner:96}.
\begin{lemme}
\label{lemme1}
Let  $T>0$ and  $N$ the integer part of  $\tfrac{T}{\Delta t}$.
We consider $\QQ \subset \R^2$, a bounded  domain.
Let 
$(\bu^h)_{h}$ be a sequence such that  $\bu^h(\; . \; ,t_n) \in X_h$ for any 
$n\leq N$. We assume 
there exists a constant  $C$ independant of  $h$ and  $\bu\in
L^{2}_{loc}(\QQ\times [0,T])$ such that 
$$
\sup_h \sup_{x,y,t}|\bu^h(x,y,t)|\leq  C ,\; \; \; \lim_h
\norm{\bu^h-\bu}_{L^2(\QQ\times [0,T])}=0.
$$
We define $$\overline{\bu^h}_K=\dfrac{1}{|K|}\int_K \bu^h\; d\bx$$
the average value of $\bu^h$ in $K$.
Then 
\begin{enumerate}
\item \begin{equation}\label{BV:1}\lim\limits_{h\rightarrow 0} \bigg (\sum\limits_{n=0}^N \Delta t \sum\limits_{K\subset \QQ} 
|K|\sum\limits_{\sigma
\in K} \norm{\bu^h_\sigma-\overline{\bu^h}_K)}\bigg )=0.\end{equation}
\item and 
\begin{equation}\label{BV:2}\lim_h h \; \norm{\nabla
{\bu}^h}_{L^2(\QQ\times [0,T])}=0.\end{equation}
\end{enumerate}
\end{lemme}

\begin{proof}
It is enough to prove the lemma for real valued functions $v$ and $(v^h)_h$ 
that satisfies the  assumptions.

\medskip

\noindent\textbf{First claim:}
We write
$v^h=\sum\limits_n\sum\limits_\sigma v^h_\sigma \varphi_\sigma\chi_{[t_n, t_{n+1}]}$ and
$$\overline{v^h}=\sum_n \sum_{K} \overline{v^h}_K \chi_{K\times [t_n, t_{n+1}]}$$ where $\chi_A$ is the characteristic function of the set $A$. These two functions are in $L^\infty (\QQ\times [0, T])$ and 
\begin{equation*}
\begin{split}
\sum\limits_{n=0}^N \Delta t \sum\limits_{K\subset \QQ} |K| \sum\limits_{\sigma
\in K} \big |v^h_\sigma-\overline{v^h}_K)\big |&\leq C_2 \sum\limits_{n=0}^N \Delta t \int_\QQ |v^h-\overline{v^h}\big |\; d\bx\\
&\leq \int_0^T \int_{\QQ}|v^h-\overline{v^h}\big |\; d\bx dt.
\end{split}
\end{equation*}


Since  $(v^h)$ is bounded, and $L^\infty (\QQ\times [0, T])\subset L^1(\QQ\times [0, T])$, there exists  $v'\in L^{\infty}(\QQ \times
[0,T])$ such that 
$v^h \rightarrow v'$ for the weak-$\star$ topology. Similarly, the exists
 $\bar v\in
L^{\infty}(\QQ\times [0,T])$, with $\overline{v^h} \rightarrow \bar v$ for the weak-$\star$ topology.

Since $v_h\rightarrow v$ in $L^2_{loc}$, we have $v'=v$ because
 $\QQ\times[0,T]$ is bounded and 
$C^{\infty}_0(\QQ\times[0,T])$ is dense in 
$L^1(\QQ\times [0,T])$.

Let us show that   $\bar v=v$. Let be  $\phi\in C^{\infty}_0(\R^2\times \R^+)$
We have, setting
$$\overline{\phi}=\dfrac{1}{|K|\Delta t}\int_{t_n}^{t_{n+1}}\int_K \phi(\bx,t)\; d\bx dt,$$
\begin{equation*}
\begin{split}
\int_0^T\int_{\QQ} \big (\overline{v^h}-v^h\big )\phi(\bx,t)\; d\bx dt&=\sum_n \sum\limits_{K, K\cap \QQ\not =\emptyset} \int_K \big (\overline{v^h}-v^h\big )\phi(\bx,t)\; d\bx dt\\
&=\sum_n \sum\limits_{K, K\cap \QQ\not =\emptyset} \bigg ( \int_K \big (\overline{v^h}-v^h\big )\phi(\bx,t)\; d\bx dt-\int_K \big (\overline{v^h}-v^h\big )\overline{\phi}\; d\bx dt\\
&=\sum_n \sum\limits_{K, K\cap \QQ\not =\emptyset} \bigg ( \int_K \big (\overline{v^h}-v^h\big )\big ( \phi(\bx,t)-\overline{\phi}\big )\; d\bx dt
\end{split}
\end{equation*}
Since $\phi\in C^{\infty}_0(\R^2\times \R^+)$, there exists $C$ that depends only on $||\nabla \phi||_{L^\infty(\R^2\times \R^+)}$ such that
$$
\bigg |\int_K \big (\overline{v^h}-v^h\big )\big ( \phi(\bx,t)-\overline{\phi}\big )\; d\bx dt\bigg |\leq \Delta t |K| \max |v^h_\sigma| \; h,$$
and then
$$\bigg | \int_0^T\int_{\QQ} \big (\overline{v^h}-v^h\big )\phi(\bx,t)\; d\bx dt\bigg | \leq C h$$ so that, passing to the limit, $\bar v=v'$.%\footnote{If one only assume that the $v^h$ are bounded, we get $\bar v$ and $v'$ and this shows that $v'=\bar v$.}.
Since a subsequence of $v^h$ converges to $v$ in $L^2$, we have $\bar v=v'=v$.


The same technique shows that  $(v_h^2)$ and $(\bar v_h^2)$ have the same weak-$\star$ limit. Let us show it is 
$v^2$. By density of 
$C^{\infty}_0(\QQ\times[0,T])$  in 
$L^1(\QQ\times [0,T])$ and since  $v_h^2$ is bounded  independently of $h$,
we may choose test functions  $\phi$ in 
$C^{\infty}_0(\QQ\times[0,T])^p$.
The function  $\phi$ is bounded in $\QQ\times[0,T]$.
Hence, we have, at least for a subsequence,
$$\int_{\QQ\times [0,T]} |v-v_h|^2 \phi dx dt \rightarrow 0,$$
and then
$$\int_{\QQ\times [0,T]} v^2 \phi dx dt -2
\int_{\QQ\times [0,T]} v v_h \phi dx dt +
\int_{\QQ\times [0,T]} v_h^2 \phi dx dt \rightarrow 0.$$
By the  Cauchy Schwarz inequality, $v \phi \in L^1(\QQ\times [0,T])$:
the second term  tends towards
$$\int_{\QQ\times [0,T]} v^2 \phi dx dt $$
and then
$$\lim\limits_{\stackrel{\text{weak}-\star}{h\rightarrow 0}}\int_{\QQ\times [0,T]} v_h^2 \phi dx dt=-\int_{\QQ\times [0,T]} v^2 \phi dx dt+2\lim\limits_{\stackrel{\text{weak}-\star}{h\rightarrow 0}} \int_{\QQ\times [0,T]} v v_h \phi dx dt 
=\int_{\QQ\times [0,T]} v^2 \phi \; d\bx dt,$$
and the  $v_h^2\rightarrow v^2$ in  $L^{\infty}$ weak-$\star$.

Last, by the same argument for  $\phi =1$, since
$w_h^2\rightarrow v^2$
in  $L^{\infty}$ weak star, we obtain
$$
\int_{\QQ\times [0,T]} |\bar v_h -v|^2 \; d\bx dt \rightarrow 0,$$
and finally,
$$
\int_{\QQ\times [0,T]} |\bar v_h -v_h|^2 \; d\bx dt \rightarrow 0.$$
Since   $\QQ\times [0,T]$ is bounded, hence  $L^1(\QQ\times [0,T]) \subset
L^2(\QQ\times [0,T]) $, we obtain \eqref{BV:1}.

\medskip

\noindent\textbf{Second claim:}
Since 
$$\nabla {v}_h^{|K} = \sum_{\sigma \in K} v^h_\sigma \nabla \varphi_\sigma=\sum_{\sigma\in K}\big ( v_\sigma -\overline{v^h}\big )\nabla \varphi_\sigma,$$
 we have
$$
\Delta t \sum\limits_{0}^N \int_{\QQ} \norm{\nabla {v}_h^n}^2\; d\bx dt
\leq C_1 \Delta t \sum\limits_0^N \sum_{K, K\subset \QQ} |K|\sum\limits_{\sigma \in K}
\big | v_{\sigma}^n-\overline{v}_K^n\big |^2 $$
because the triangulation is regular (assumption  \ref{H0}).
We conclude by the same arguments as before.
\end{proof}

\begin{lemme}
\label{lemme2}
Let $\varphi \in C_0^{k+1}(\R^2 \times \R^+)$. With the assumptions of 
Theorem
\ref{th1}, one has
$$ \sum\limits_n\Delta t \sum\limits_\sigma |C_\sigma| \big (u^{n+1}_{\sigma}-u^n_{\sigma} \big ) \varphi(\sigma,t_n)+
\int_{\R^2\times \R^+} u \dpar{\varphi}{t} dx dt +\int_{\R^2} u_0(x)
\varphi(x,0)\rightarrow 0$$
when $h \rightarrow 0$.
\end{lemme}
The proof is classical: it is the same as in the proof of the classical
 Lax Wendroff theorem.

Let us introduce $\psi_\sigma$ the basis function at $\sigma$ and $\Psi_\sigma^K$, $\Psi_\sigma^{K'_K}$  the residuals
$$
\Psi_\sigma^K=-\int_{K} \nabla \varphi_\sigma \bbf^h(\bu^h)+\int_{\partial K} \varphi_\sigma \bbf^h(\bu^h)\cdot \bn \; d\gamma.
$$
It is clear that
$$\sum_{\sigma \in K} \Psi_\sigma^K=\int_{\partial K}\bbf^h(\bu^h)\cdot \bn \; d\gamma=\sum_{\sigma \in K} \Phi_\sigma^K.$$
We have
\begin{lemme}
\label{lemme3}
Let $\varphi \in C^{k+1}_0(\R^2\times \R^+)$, $\bbf\in
(C^{1}(\R^m))^{d}$, $d=2$. Assume that
 $f^h$ satisfies the assumption
  \ref{H2}--{\it (iii)},  and that  $\bu_h$ satisfies those of Theorem 
 \ref{th1}. Then
$$
\Delta t   \sum\limits_{n,K}\sum\limits_{\sigma \in K'_K \subset K} \varphi_\sigma^n
\Phi_{\sigma}^{K} (\bu_h^n)
+
\int_{R^2\times \R^+} \nabla \varphi(\bx,t)\cdot \bbf(\bu(\bx,t))  \; d\bx dt \rightarrow 0$$
when $h \rightarrow 0$.
\end{lemme}


\begin{proof}
Let $\varphi\in C_0^1(\R^2 \times [0,+\infty[)$. Let $\Omega$ and $T$
such that 
$\text{supp}(\varphi) \subset \Omega \times [0,T]$. Consider $K \in
\TT_h$ 
Now $\pi_h^k \varphi$ is the interpolation of $\varphi$ of degree $k$. We have:
$$
\Delta t \sum_{n,K}  \sum_{\sigma \in K} \varphi_\sigma^n
\Psi_{\sigma}^{K} (\bu_h^n) =
\sum_{n,K} \int_{t^n}^{t^{n+1}} \int_K\nabla\pi_h^k \varphi(\bx,t_n) \cdot \bbf^h_K (\bu_h^n) \; d\bx dt
$$ 
since  
\begin{equation*}
\begin{split}
 \sum_{\sigma\in K}  \varphi_\sigma^n \Psi_{\sigma}^{K} (\bu_h^n)&=
-\sum\limits_K \int_K \nabla(\pi_h^k \varphi)(x,t_n) \; . \; \bbf^h_K(\bu_h^n) dx +  \int_{\partial K}
\pi_h^k \varphi(x,t^n) \bbf_K^h(\bu_h^n)\; . \bn d\bx.
\end{split}\end{equation*}
By continuity of $\bu_h^n$ and $\pi_h^k\varphi$, the boundary terms cancel.
.

Moreover,  $\varphi$ is $C^{k+1}$ and the triangulation is regular~:
 $\nabla (\pi_h^k \varphi)$ is uniformly bounded by a constant $C$ 
independant of $h$.
Thus we have
\begin{equation*}
\begin{split}
\bigg |\sum\limits_{n,K}& \int_{K\times [t_n,t_{n+1}]} \nabla(\pi_h^k
\varphi)(\bx,t_n) \;
. \; \bbf^h_K(u_h^n) \; d\bx dt- \sum\limits_{n,K} \int_{K\times [t_n,t_{n+1}]} \nabla \varphi \; . \; \bbf(u) \; d\bx dt \bigg |\\
&\leq  C  \sum \limits_{n,K}\int_{K\times[t^n,t^{n+1}]} \norm{\bbf^h(\bu_h)-\bbf(\bu)} \; d\bx  dt + \sum\limits_{n,K}\int_{K\times[t^n,t^{n+1}]} \norm{\nabla \pi_h^k\varphi-\nabla \varphi} \; \norm{\bbf(\bu_h)}\;dx dt
 \end{split}\end{equation*}
The first sum is less than
$\norm{\bbf^h(\bu_h)-\bbf(\bu)}_{L^1(\text{supp }\varphi \times [0,T])}\leq C_\bbf ||\bu_h-\bu||_{L^1(\text{supp }\varphi \times [0,T])}$
and tends to  $0$ because  $\norm{u_h}_{\infty}$ is bounded independantly of
 $h$, 
 $\bbf$ is  $C^1$ and $\bu_h \rightarrow \bu$ in  $L^2_{loc}$.

Similarly, since  $\bu_h$ is bounded and  $f$ is continuous, $\bbf(\bu_h)$ is bounded
uniformly in $h$ by a constant $C$.
The second term of the right hand side sum is bounded by the $L^1$ norm of 
 $\nabla \pi_h^k\varphi-\nabla \varphi$ that
tends to $0$ since the triangulation is uniform.

\end{proof}

%%
\begin{proof}[Proof of  Th{e}or{e}m \ref{th1}:] We multiply
 ({\ref{leschema}})
by $\varphi_\sigma^n |C_\sigma|$, where  the test function $\varphi $
belongs to  $ C^{k+1 }_0\left( {\R}^2 \times [0,+\infty [ \right)$, such that
$\text{supp}(\varphi ) \subset \Omega \times [0,T]$ for  $\Omega$ and
$K$ well chosen ($n \Delta t \leq T$). Then we sum up on $J$ the set of $(\sigma,t_n)$  such that
   $(\sigma,t_n)\in
\Omega \times [0, T] $:
%%
\[
 \sum\limits_{(\sigma,t_n)\in J}  |C_\sigma| \left(
\bu^{n+1}_{\sigma} - \bu^n_\sigma\right) \varphi_\sigma^n \; + \;
\Delta t \sum\limits_{(\sigma,t_n)\in J} 
 \sum\limits_{ \sigma \in K} \Phi^{K}_\sigma(\bu_h^n) \varphi_\sigma^n
 = 0,
\]
From Lemma \ref{lemme2}, we have
\[
\sum\limits_{(\sigma,t_n)\in J}  |C_\sigma| \left(
\bu^{n+1}_\sigma - \bu^n_\sigma \right) \varphi_\sigma^n =
  \int_{ {\R}^2 \times {\R}^+ } \bu \dpar{ \varphi}{t}\; d\bx dt
 - \int _{{\R}^2} \bu_0 \varphi(~.~,0) \; d\bx+ o(1).
\]
For the space term, we write:
\begin{equation*}
\begin{split}
 \sum\limits_{(\sigma,t_n)\in J}  \sum\limits_{K; \sigma \in K}
\Phi_\sigma^{K,n} \varphi_\sigma^n & =
\sum_{K\subset \Omega } \bigg(
\sum\limits_{\sigma \in  K} \varphi_\sigma^n \big (\Phi_{\sigma}^{K,n}-\Psi_{\sigma}^{K,n} \big ) \bigg  )+ \sum\limits_{K\subset \Omega }\sum_{\sigma \in  K} \varphi_\sigma^n\Psi_{\sigma}^{K,n}
,
\end{split}
\end{equation*}
By the conservation relation, we have
$$
\sum_{\sigma \in K} \big (\Phi_{\sigma}^{K,n}-\Psi_{\sigma}^{K,n} \big )=0, 
$$
so introducing $\overline{\varphi}_K$ the average of $\pi_k^h\varphi$ in  $K$ and  $\Phi_{\sigma}^{K,n}-\Psi_{\sigma}^{K,n}=\SS_\sigma^{K,n}$
to simplify, 
\begin{equation*}\begin{split}
\sum\limits_{\sigma \in K} \varphi_\sigma^n  \SS_\sigma^{K,n}&=
\sum\limits_{\sigma \in K} \varphi_\sigma^n  
\SS_\sigma^{K,n}-\overline{\varphi}_K
\sum\limits_{\sigma \in K}\SS_\sigma^{K,n}= \sum\limits_{\sigma \in K}\big (\varphi_\sigma^n- \overline{\varphi}_K\big )
\SS_\sigma^{K,n}.
\end{split}
\end{equation*}

By  Lemma \ref{lemme3}, we have
\[
\Delta t  \sum\limits_{n=0,N} 
 \sum\limits_{\sigma\in J} \sum\limits_{K; \sigma \in K}
\Phi_\sigma^{K,n} \varphi_\sigma^n
 = -  \int _{ {\R}^2 \times {\R}^+ } \bbf(\bu({\bx},t))\cdot \nabla
 \varphi ({\bx},t)\; d{\bx}dt \; + \; o(1).
\]
%%  
Last, from assumption \ref{H3} and Lemma
\ref{lemme1}, we have
\begin{equation*}
\begin{split}
 \Delta t \norm{ \sum_{n,K} 
\sum\limits_{\sigma  \in K}\SS_\sigma^{K,n}
    \big (\varphi_\sigma^n-\varphi_\sigma^n \big )}
    & \leq C h \Delta t \sum\limits_{n=0,N}  \sum\limits_{K\subset \Omega }
\norm{\SS_{\sigma}^K(\bu_h^n) }
 \\
    & \leq C h^2 \Delta t
 \sum\limits_{n=0,N}  \sum\limits_{K\subset \Omega }
   \sum\limits_{\sigma\in K}
 \norm{\bu^n_\sigma - \overline{\bu^h}_K}
     \longrightarrow 0,
\end{split}
\end{equation*}
because both $\Psi_\sigma$ and $\Phi_\sigma$ satisfy assumption \ref{H3}.
This ends the proof
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%


==> correctum.tex <==
Hence, \eqref{momentum:1} can be rewritten as:
\begin{equation}
\label{momentum:2}
\begin{split}
\int_{\R^d}&\psi(\bx,t) \; \big ( \rho^{{n+1}}\bu^{{n+1}}-\rho^{{n}}\bu^{{n}}\big ) \; d\bx\\
& =\sum_K\psi_K^n\bigg [\sum_{\sigma_{\mathcal{V}}\in K} \Delta \bu_{\sigma_\mathcal{V}}\int_K \rho^{{n+1}}\varphi_{\sigma_\mathcal{V}}\; d\bx+ \sum_{\sigma_{\mathcal{E}}\in K}\Delta \rho_{\sigma_{\mathcal{E}}}\int_K \bu^{{n}}\varphi_{\sigma_\mathcal{E}}\; d\bx
\bigg ]\\
&\quad=\sum_K\psi_K^n\bigg [\sum_{\sigma_{\mathcal{V}}\in K} \omega^{\rho,n+1,K}_{{\sigma_{\mathcal{V}}}} 
|C_{\sigma_{\mathcal{V}}}|\Delta \bu_{\sigma_\mathcal{V}}
 + \sum_{\sigma_{\mathcal{E}}\in K}\omega^{\bu,n,K}_{\sigma_\mathcal{E}}
|C_{\sigma_\mathcal{E}}|\Delta \rho_{\sigma_{\mathcal{E}}}\bigg ]\\
&=\sum_K\Big [\sum_{\sigma_\V\in K} \psi_{\sigma_\V}\omega_{\sigma_\V}^{\rho, n+1,K}|C_{\sigma_{\mathcal{V}}}|
\Delta \bu_{\sigma_\mathcal{V}} \Big ]\\
&\qquad +
\sum_K\sum_{\sigma_\V} \big (\psi_K^n-\psi_{\sigma_\V}\big )\vert C_{\sigma_{\mathcal{V}}}\vert \; \omega_{\sigma_\V}^{\rho, n+1}
\Delta \bu_{\sigma_\mathcal{V}}+\sum_K \psi^n_K \Big [\sum_{\sigma_{\mathcal{E}}\in K}\omega^{\bu,n,K}_{\sigma_\mathcal{E}}
|C_{\sigma_\mathcal{E}}|\Delta \rho_{\sigma_{\mathcal{E}}}\Big ]\\
&=
\sum_{\sigma_\V} \psi_{\sigma_\V}^n \omega_{\sigma_\V}^{\rho, n+1}\vert C_{\sigma_{\mathcal{V}}}\vert \;\Delta \bu_{\sigma_\V} +
\sum_K\sum_{\sigma_\V\in K} \big (\psi_K^n-\psi_{\sigma_\V}\big )\vert C_{\sigma_{\mathcal{V}}}\vert \; \omega_{\sigma_\V}^{\rho, n+1}
\Delta \bu_{\sigma_\mathcal{V}}
\\
&\qquad+\sum_K \psi^n_K \Big [\sum_{\sigma_{\mathcal{E}}\in K}\omega^{\bu,n,K}_{\sigma_\mathcal{E}}|C_{\sigma_\mathcal{E}}|\Delta \rho_{\sigma_{\mathcal{E}}}\Big ]
\end{split}
\end{equation}
where we have set for simplicity
$$\omega^{\rho,n+1,K}_{{\sigma_{\mathcal{V}}}}:=\dfrac{\int_K \rho^{{n+1}}\varphi_{\sigma_\mathcal{V}}\; d\bx}{|C_{\sigma_{\mathcal{V}}}|}\; \text{ , }\;
\omega^{\bu,n,K}_{\sigma_\mathcal{E}}:=\dfrac{\int_K \bu^{{n}}\varphi_{\sigma_\mathcal{E}}\; d\bx}{|C_{\sigma_\mathcal{E}}|}$$
and (using that the support of $\varphi_{\sigma_\V}$ is the union of the elements that share $\sigma_\V$),
$$\omega^{\rho,n+1}_{{\sigma_{\mathcal{V}}}}:=\dfrac{\int_\Omega \rho^{{n+1}}\varphi_{\sigma_\mathcal{V}}\; d\bx}{|C_{\sigma_{\mathcal{V}}}|}$$

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.45\textwidth]{stencilD.pdf}
\end{center}
\caption{\label{stencilD} For an element $K$ (shaded region) and any one of the degrees of freedom $\bullet$, the  $\square$ represent the elements $K'$ that come in the sum \eqref{momentum:3} and the definition of $\mathcal{D}$ of \eqref{eq:D}.}
\end{figure}

For the velocity, we have:
$$|C_{\sigma_{\mathcal{V}}}|\big ( \bu_{\sigma_\mathcal{V}}^{{n+1}}-\bu^{{n}}_{\sigma_\mathcal{V}}\big ) +\Delta t_n\sum_{K, \sigma_\mathcal{V}\in K}\Phi^\bu_{\sigma_\mathcal{V},K}=0,$$
where, for the forward Euler scheme \eqref{forw_Euler}, 
$$\Phi^\bu_{\sigma_\mathcal{V},K}=\Phi^\bu_{\sigma_\mathcal{V},K}(U^{{n}}
\big ).$$
%************************************************** 

%************************************************** 
For the density, we have
$$\vert C_{\sigma_\mathcal{E}}\vert \big ( \rho_{\sigma_{\mathcal{E}}}^{{n+1}}-\rho_{\sigma_{\mathcal{E}}}^{{n}}\big ) +\Delta t_n
\sum_{K, \sigma_{\mathcal{E}}\in K} \Phi_{\sigma_{\mathcal{E}},K}^{\rho}=0$$
and we note that the sum reduces to one term, hence
$$\vert C_{\sigma_\mathcal{E}}\vert \big ( \rho_{\sigma_{\mathcal{E}}}^{{n+1}}-\rho_{\sigma_{\mathcal{E}}}^{{n}}\big ) +\Delta t_n 
\Phi^\rho_{\sigma_{\mathcal{E}},K}=0,$$
where again
$$\Phi^\rho_{\sigma_{\mathcal{E}},K}=\Phi^\rho_{\sigma_\mathcal{E},K}(U^{{n}})$$and $K$ is \emph{the} element such that $\sigma_\mathcal{E}\in K.$
%************************************************** 
Using these relations in \eqref{momentum:2}, we get
\begin{equation}
\label{momentum:3}
\begin{split}
\int_{\R^d}&\psi(\bx,t) \; \big ( \rho^{{n+1}}\bu^{{n+1}}-\rho^{{n}}\bu^{{n}}\big ) \; d\bx+\Delta t_n\underbrace{
\sum_{\sigma_\V} \psi_{\sigma_\V}^n \omega_{\sigma_\V}^{\rho, n+1}
\bigg [ \sum_{K, \sigma_\V\in K}\Phi^\bu_{\sigma_\bV,K}\bigg ]}_{I}\\&
+
\Delta t_n\sum_K\bigg \{\sum_{\sigma_\V\in K} \big (\psi_K^n-\psi_{\sigma_\V}\big )\omega_{\sigma_\V}^{\rho, n+1,K}\Big [ \sum_{K', \sigma_\bV\in K'\cap K} \Phi^\bu_{\sigma_b,K}\Big ]\bigg \}
\\
&\qquad+
\Delta t_n\sum_K \psi^n_K \Big [\sum_{\sigma_{\mathcal{E}}\in K}\omega^{\bu,n,K}_{\sigma_\mathcal{E}}\Phi^\rho_{\sigma_\E,K}\Big ]
\\
&\qquad\qquad=0
\end{split}
\end{equation}
The term $I$ can be rewritten as 
\begin{equation*}
\begin{split}
\sum_{\sigma_\V} &
\psi_{\sigma_\V}^n \omega_{\sigma_\V}^{\rho, n+1}
\bigg [ \sum_{K, \sigma_\V\in K}\Phi^\bu_{\sigma_\bV,K}\bigg ]=
\sum_{K} \psi^n_K \sum_{\sigma_\V\in K} \omega_{\sigma_\V}^{\rho, n+1}\Phi^\bu_{\sigma_\bV,K}\\
&\qquad 
+
\sum_K \bigg [ \sum_{\sigma_\V\in K} \big ( \psi^n_K-\psi^n_{\sigma_\V}\big )\omega_{\sigma_\V}^{\rho, n+1}\Phi^\bu_{\sigma_\bV,K}
\bigg ]
\end{split}
\end{equation*}
Hence, gathering all together, we get
\begin{equation*}
\begin{split}
\int_{\R^d}&\psi(\bx,t) \; \big ( \rho^{{n+1}}\bu^{{n+1}}-\rho^{{n}}\bu^{{n}}\big ) \; d\bx\\
 &+\Delta t_n
\sum_{K} \psi^n_K\Bigg [  \sum_{\sigma_\V\in K} \omega_{\sigma_\V}^{\rho, n+1}\Phi^\bu_{\sigma_\bV,K}
\sum_{\sigma_{\mathcal{E}}\in K}\omega^{\bu,n,K}_{\sigma_\mathcal{E}}\Phi^\rho_{\sigma_\E,K}\Bigg ]\\\qquad &
+\Delta t_n
\sum_K \bigg [ \sum_{\sigma_\V\in K} \big ( \psi^n_K-\psi^n_{\sigma_\V}\big )\omega_{\sigma_\V}^{\rho, n+1}\Phi^\bu_{\sigma_\bV,K}
\bigg ]\\
&\qquad \qquad
+\Delta t_n
\sum_K\bigg \{\sum_{\sigma_\V\in K} \big (\psi_K^n-\psi_{\sigma_\V}\big )\omega_{\sigma_\V}^{\rho, n+1,K}\Big [ \sum_{K', \sigma_\bV\in K'\cap K} \Phi^\bu_{\sigma_b,K}\Big ]\bigg \}=0
\end{split}
\end{equation*}

Thus, we obtain the master equation:
\begin{subequations}
\begin{equation}
\label{master:1}
\begin{split}
 \int_{\R^d}\psi(\bx,t) \; &\big ( \rho^{{n+1}}\bu^{{n+1}}-\rho^{{n}}\bu^{{n}}\big ) \; d\bx 
 \\&+\Delta t\sum_K \psi_K^n \Bigg [ 
\sum_{\sigma_\mathcal{V}\in K} \omega^{\rho,n+1}_{\sigma_\mathcal{V}} \Phi_{\sigma_\mathcal{V},K}^\bu 
+\sum_{\sigma_{\mathcal{E}}\in K}\omega^{\bu,n,K}_{\sigma_\mathcal{V}}
\Phi^\rho_{\sigma_{\mathcal{E}},K}
 \Big ]\\
%&\qquad \qquad \qquad
&\qquad+ \Delta t_n
\sum_{K}\Big ( {F}_K^\bm+ D_K^\bm%\sum_{\sigma_\mathcal{V}\in K}D^K_{\sigma_\mathcal{V}}
\Big )=0
\end{split}
\end{equation}
with {\color{red}
\begin{equation}
\label{master:2}
\begin{split}
F_K^\bm&=\sum_{\sigma_\V\in K} \big ( \psi^n_K-\psi^n_{\sigma_\V}\big )\omega_{\sigma_\V}^{\rho, n+1}\Phi^\bu_{\sigma_\V,K}\\
D_{K}^\bm&=\sum_{\sigma_\V\in K} \big (\psi_K^n-\psi_{\sigma_\V}\big )\omega_{\sigma_\V}^{\rho, n+1,K}\Big [ \sum_{K', \sigma_\bV\in K'\cap K} \Phi^\bu_{\sigma_b,K}\Big ]\\
%\sum_{\sigma_\mathcal{V}\in K}\big ( \psi^n_K-\psi^n_{\sigma_\V}\big )\omega_{\sigma_\V}^{\rho, n+1}\Phi^\bu_{\sigma_\V,K} \\
 \omega_{\sigma_\V}^{\rho,n+1,K}&=\dfrac{ \int_K \rho^{{n+1}}\varphi_{\sigma_\mathcal{V}}\; d\bx}{\vert C_{\sigma_\mathcal{V}}\vert}, \qquad
\omega_{\sigma_\mathcal{V}}^{\rho,n+1}=
\sum\limits_{K, \sigma_\V\in K}\omega_{\sigma_\mathcal{V}}^{\rho,n+1,K}
\\
\omega^{\bu,n,K}_{\sigma_\mathcal{E}}&=\dfrac{\int_K \bu^{{n}}\varphi_{\sigma_\mathcal{E}}\; d\bx}{\vert C_{\sigma_\mathcal{E}}\vert}. 
\end{split}
\end{equation}  }
\end{subequations}


